MaPa: Text-driven Photorealistic Material Painting for 3D Shapes

This paper aims to generate materials for 3D meshes from text descriptions. Unlike existing methods that synthesize texture maps, we propose to generate segment-wise procedural material graphs as the appearance representation, which supports high-quality rendering and provides substantial flexibility in editing. Instead of relying on extensive paired data, i.e., 3D meshes with material graphs and corresponding text descriptions, to train a material graph generative model, we propose to leverage the pre-trained 2D diffusion model as a bridge to connect the text and material graphs. Specifically, our approach decomposes a shape into a set of segments and designs a segment-controlled diffusion model to synthesize 2D images that are aligned with mesh parts. Based on generated images, we initialize parameters of material graphs and fine-tune them through the differentiable rendering module to produce materials in accordance with the textual description. Extensive experiments demonstrate the superior performance of our framework in photorealism, resolution, and editability over existing methods. Project page: https://zju3dv.github.io/MaPa

==> 04_experiments.tex <==

\section{Experiments}

\subsection{Implementation details}
% 我们的three stages的material graph optimization都使用adam作为优化器。第一个stage我们优化200个iterations，
Our material graph optimization in three stages uses Adam~\cite{kingma2014adam} as the optimizer. We perform a total of 300 iterations for optimization. %Therefore, the overall algorithm does not take a long time to run.
% 一般来讲在一张A6000上面完成算法的整个流程需要不到10分钟。
In general, the entire process of our method can be completed in less than 10 minutes on an A6000, which is faster than Text2tex~\cite{chen2023text2tex} (15 minutes) and Fantasia3D~\cite{Chen_2023_ICCV} (25 minutes).
% 我们收集了9个material类别，包括：wood, metal, plastic, leather, fabric, glass, stone, ceramic, rubber。其中的每个类别的个数由表格~\ref{tab:dataset}~\tocite{}给出。
We collect 8 material categories, including wood, metal, plastic, leather, fabric, stone, ceramic, and rubber. The number of each category is given in the supplementary material.
% 对于透明材质，我们只进行retrieve，不进行optimize。
% For transparent materials, we only perform retrieve without optimization.

\subsection{Comparison to baselines}
\paragraph{Baselines.}
We compare our method with three strong baselines on text-driven appearance modeling.
% 2. TEXTure~\cite{richardson2023texture} introduces an iterative texture painting scheme to generate texture maps for 3D objects.
TEXTure~\cite{richardson2023texture} introduces an iterative texture painting scheme to generate texture maps for 3D objects.
% 3. Text2tex~\cite{chen2023text2tex} uses a similar scheme to TEXTure. Additionally, it creates an automated strategy for selecting viewpoints during the iterative process.
Text2tex~\cite{chen2023text2tex} uses a similar scheme to TEXTure. Additionally, it creates an automated strategy for selecting viewpoints during the iterative process.
% 对于下面的实验，We use a environmental map to render results of our method and Fantasia3D. Results of TEXTure and Text2tex are obtained by their diffuse color pass in Blender.
Fantasia3D~\cite{Chen_2023_ICCV} separates the modeling of geometry and appearance, adopting an MLP to model the surface material properties of a 3D object.
For the following experiments, we employ an environmental map to generate outcomes for our method and Fantasia3D. The results for TEXTure and Text2tex are derived from their diffuse color pass in Blender.


\input{tab/comtab.tex}



%\subsection{Quantitative evaluation}
\paragraph{Quantitative comparison.}
Our goal is to obtain high rendering quality that is as close as possible to the real image, so we measure the distribution distance between the rendered image and the real image using FID~\cite{heusel2017gans} and KID~\cite{binkowski2018demystifying}.
%are used as our quantitative metrics.
However, it is difficult to obtain a large number of high-quality 3D shapes and real images simultaneously. Therefore, we only select the chairs dataset from TMT~\cite{hu2022photo} as our test data. 300 chairs are selected as test data, and 10 views are uniformly sampled for each chair with a 360-degree azimuth range, a constant 45-degree elevation angle, and a fixed radius of 1.5 units. 
The prompt in the experiment is extracted from the chairs dataset~\cite{hu2022photo} using BLIP~\cite{li2022blip}. 
Each baseline uses the same prompts.
The segmentation of the each input shape is obtained by finding connected components.

Moreover, we also conducted a user study to assess the rendering results. 
Each respondent was asked to evaluate the results based on two aspects: overall quality and fidelity to the text prompt, using a scale of 1 to 5. 
Overall quality refers to the visual quality of the rendering results, while fidelity to the text prompt indicates how closely these results align with the given text prompt.
There were 40 users participated in the study, including 16 professional artists and 24 members of the general public. We gathered 60 responses from each participant, and the final score represents the average of all these responses.
As shown in Table~\ref{tab:quantitative}, our method achieves the best quantitative results and the highest user study scores.

\paragraph{Qualitative comparison.}
We collect several high-quality 3D models from Sketchfab~\cite{sketchfabSketchfabBest} and use these data for qualitative experiments. 
As shown in Figure~\ref{fig:qualitative}, our method can achieve more realistic rendering results than the baselines.
TEXTure and Text2tex are prone to produce inconsistent textures, which makes their results look dirty.      
Fantasia3D's results frequently exhibit oversaturation or fail directly.

% \input{contents/comparsion/comparisons.tex}

\input{contents/diversity/diversity.tex}



\subsection{More qualitative results}

%\paragraph{Visual comparison to baselines.}



\paragraph{Diversity of results.}
2D diffusion model can generate different images with different seeds, which naturally brings diversity to our framework when optimizing material according to the generated images.
We show an example shape with diverse results in Figure~\ref{fig:diversity}. 
Note how the painted materials change when different images of the same object are generated.
%我们渲染的结果可以符合生成的图片，因此我们的方法可以产生多样的结果。
%\zsz{We use the same prompt but different seeds to generate different images. Our rendering results can match the generated images, so our method can produce diverse results.}
%\rh{[add a few sentence to describe the results.]}

\paragraph{Appearance transfer from image prompt.}
% 如果我们使用the image encoder introduced in IP-Adapter~\cite{ye2023ip-adapter}兼容Image Prompt, 我们的方法就可以做appearance transfer。
We can use the image encoder introduced in IP-Adapter~\cite{ye2023ip-adapter} to be compatible with image prompt. 
As shown in Figure~\ref{fig:reference}, our method can transfer the appearance from the reference image to the input objects by first generating the corresponding image of the given object with similar appearance and then optimizing the materials using our framework.





\input{contents/reference/reference.tex}



%\subsection{More results}
\paragraph{Results on watertight meshes.}
% 虽然我们主要focus在能被连通算法分割的mesh上，但是我们的方法也可以处理watertight mesh。在图中，我们同时展示了编辑watertight mesh的结果。我们利用graph cut算法分割了watertight mesh，然后我们为每个segment生成了材质。
Although we mainly focus on meshes that can be segmented by grouping connected components, our method can also handle watertight meshes. In Figure~\ref{fig:wtm}, we also show the results of painted watertight meshes. We use the graph cut algorithm~\cite{katz2003hierarchical} to segment the watertight mesh, and then we generate materials for each segment.




\paragraph{Downstream editing results.}
% % 我们的方法可以通过用户输入的prompt编辑高质量的纹理。在图中，我们分别输入了“增加swirling and curling patterns intertwining in a fluid纹理“， “增加纹理with pattern exudes a modern, abstract feel“ and “增加interlocking hexagons pattern在这个纹理上“。
Our method can edit materials based on user-provided prompts, and we show several editing results on a bag in Figure~\ref{fig:editing_bag}. We can see that we are able to add different patterns to the bag according to the prompts.
% \rh{[replace examples with vase, bag, and some other categories; describe the results]}




\subsection{Ablation studies}
% Segments-controlled image generation的重要性

\paragraph{The significance of albedo estimation network.}
To justify the usage of our albedo estimation network, we compare with the setting ``w/o Albedo'', where we remove this module from our method and use the generated image directly.
%We conduct an ablation study on our albedo estimation network.
%A baseline ``w/o albedo'' is the same as our method except that we do not use the albedo estimation network. 
As illustrated in Figure~\ref{fig:ablation_albedo}, the baseline ``w/o Albedo'' fails to merge the segments with the similar color, hindered by the impacts of shadow and lighting.
Additionally, a noticeable color disparity exists between the rendering result of ``w/o Albedo'' and the generated image.

\paragraph{Robustness analysis of grouping results.}
% 我们的方法即使没有material grouping也可以work，只是速度会变慢。我们在这里展示了我们的方法在没有material grouping的情况下优化的结果。我们将这个baseline简写成``w/o grouping''。 如图Figure~\ref{fig:ablation_albedo}，``w/o grouping''的结果和我们的结果相比，并没有明显的效果变差。
Our method can also work without material grouping. We show the results of our method without material grouping in Figure~\ref{fig:ablation_albedo}, referred as ``w/o Grouping''. The results of ``w/o Grouping'' are not significantly different from our results. 
However, the optimization time will be much longer without grouping. 
%We collect 30 models from Sketchfab and use these data to evaluate optimization time. 
We find our method takes 7 minutes on average to finish the all optimization process per shape. If we remove the material grouping, the optimization time on average
will increase to 33 minutes.


\input{contents/watertight/wtm.tex}

\paragraph{The significance of material graph optimization.}
We also show some representative visual comparisons with the setting ``w/o Opt'', where the material graph is selected without further optimization in Figure~\ref{fig:ablation_wood}.
We can clearly see that the optimization highly increases the appearance similarity to the generated images and is not limited by the small material graph data set.
% Generated image (a) generated image (b) and generated image (c)，在同一个pose下。
% 并且图中的wood material graph的retrival结果是一样的。这证明了即使我们的material graph data set很小，我们的方法也可以产生多样的结果。
Generated images (a), (b), and (c) are generated under the same pose. The retrieval results of the wood material graph in the three images are the same shown as ``w/o Opt''. This proves that even if our material graph data set is small, our method can still produce diverse texture results.
% 我们还消融实验了我们的residual lighting。我们的方法在没有residual lighting的情况下，会产生与图片不一致的纹理。这是因为初始化的2D spatially-varying lighting不是很好，导致了我们的方法在没有residual lighting的情况下，尤其是他没有在diffusion model产生的图片数据集上训练过，有domain gap。我们将这个baseline简写成``w/o residual light''。
We also conduct an ablation study on effectiveness of residual lighting, refereed as ``w/o Res''.
Compared to our result (a), ``w/o Res'' produces textures that are inconsistent with the generated images. This is because the initial 2D spatially-varying lighting is not very accurate, which is caused by the domain gap between the training data of InvRenderNet and the images generated by the diffusion model. %We refer to this baseline as ``w/o Res''.
%\zsz{% Generated images (a) is used to 被使用来优化baseline ``w/o Opt''和``w/o Res''。
%Generated image (a) is used to optimize the baseline ``w/o Opt'' and ``w/o Res''.}



\input{contents/ablation_wood/ablation_wood.tex}
\input{contents/albation_albedo/ablation_ab.tex}
\input{contents/editing/editing_bag.tex}
\input{contents/failure/failure.tex}


%\paragraph{The significance of material graph optimization strategy.} 


==> contents/ablation_wood/ablation_wood.tex <==
\begin{figure*}
\begin{center}
\iffalse
\setlength\tabcolsep{0.2em}
\newcommand{\mywidth}{0.22 \textwidth}
\begin{tabular}{cccc}
\includegraphics[width=\mywidth]{contents/ablation_wood/input_mesh.png}
&\includegraphics[width=\mywidth]{contents/ablation_wood/diffusion4.png}
&\includegraphics[width=\mywidth]{contents/ablation_wood/diffusion4_with_env_light.png}
&\includegraphics[width=\mywidth]{contents/ablation_wood/without_env_light5.png}

\\
Input Mesh
&
Generated Image
&
Our result
& 
Ours w/o residual light

\\
\includegraphics[width=\mywidth]{contents/ablation_wood/diffusion1.png}
&\includegraphics[width=\mywidth]{contents/ablation_wood/render1.png}
&\includegraphics[width=\mywidth]{contents/ablation_wood/diffusion2.png}
&\includegraphics[width=\mywidth]{contents/ablation_wood/render2.png}
\\
Generated Image 2
&
Rendering Result 2
& 
Generated Image 3
&
Rendering Result 3
\\
\includegraphics[width=\mywidth]{contents/ablation_wood/without_optimize1.png}
\\
Ours w/o opt
\end{tabular}
\fi 
\includegraphics[width=.9\linewidth]{contents/ablation_wood/graph-optim.pdf}
\vspace{-1em}
\end{center}

\captionsetup{font={normalsize}} 
\caption{\textbf{Ablation study of our material graph optimization.}
We show the ablation study of our material graph optimization and the effectiveness of residual light.
The baseline ``w/o Opt'' and ``w/o Res'' are optimized to minimize the loss of the generated image (a) and the rendered image.
The generated image (b) and (c) are used to prove that our method can yield diverse results even with a small material graph dataset.
}
\label{fig:ablation_wood}
\end{figure*}

    


==> contents/albation_albedo/ablation_ab.tex <==

    

\begin{figure}
\begin{center}
\includegraphics[width=\linewidth]{contents/albation_albedo/fig-abg.pdf}
\vspace{-1em}
\end{center}

% \captionsetup{font={normalize}} 
\caption{\textbf{Ablation study of ``w/o Albedo'' and ``w/o Grouping''.}
The baseline ``w/o Albedo'' exhibits color disparity between the rendering result and generated image, and fails to merge segments with similar color.
The baseline ``w/o Grouping'' has similar rendering results to our method.
}
\label{fig:ablation_albedo}
\end{figure}



==> contents/closeup/closeup.tex <==
\begin{figure}
\setlength\tabcolsep{0.2em}
\newcommand{\mywidth}{0.45\textwidth}
\begin{tabular}{cc}
\includegraphics[width=\mywidth]{contents/closeup/0415.pdf}
% &\includegraphics[width=\mywidth]{contents/closeup/chair_close_up.png}
% \\
% \includegraphics[width=\mywidth]{contents/closeup/purse.png}
% &\includegraphics[width=\mywidth]{contents/closeup/purse_close_up.png}
\end{tabular}
\vspace{-1em}
\caption{\textbf{Close-up rendering results.}
Our generated material has rich details.}
\label{fig:closeup}
\end{figure}

    


==> contents/comp.tex <==
\begin{figure*}[htb]
\centering
% \begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=0.9 \textwidth]{contents/comp.pdf}
% \caption{\textbf{Qualitative comparisons.} 
% The results generated by our method and all the baselines are rendered in the same CG environment for comparison. The prompts for the three objects are: "a photo of a wooden bedside table," "a photo of a toy rocket," and "a photo of a brand-new sword."
% }
% \label{fig:qualitative}
% \label{fig:exp}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.49\textwidth}
% \newcommand{\mywidth}{0.3 \textwidth}

% \begin{tabular}{ccc}
% \includegraphics[width=\mywidth]{contents/restrictive/fanta_nightstand.png}
% &\includegraphics[width=\mywidth]{contents/restrictive/text2tex_nightstand.png}
% &\includegraphics[width=\mywidth]{contents/restrictive/Texture_nightstand.png}
% \\
% Fantasia3D
% &
% Text2tex
% & 
% TEXTure
% \\
% \includegraphics[width=\mywidth]{contents/restrictive/fanta_rocket.png}
% &\includegraphics[width=\mywidth]{contents/restrictive/text2tex_rocket.png}
% &\includegraphics[width=\mywidth]{contents/restrictive/Texture_rocket.png}
% \\
% Fantasia3D
% &
% Text2tex
% & 
% TEXTure
% \\
% \includegraphics[width=\mywidth]{contents/restrictive/fanta_sword.png}
% &\includegraphics[width=\mywidth]{contents/restrictive/text2tex_sword.png}
% &\includegraphics[width=\mywidth]{contents/restrictive/Texture_sword.png}
% \\
% Fantasia3D
% &
% Text2tex
% & 
% TEXTure

% \end{tabular}
% \vspace{-1em}
% \caption{\textbf{Restrictive prompts.} 
% \revise{We use more restrictive prompts to guide the baselines, adding ``with uniform color'' to each prompt. 
% The results show that the baselines are still unable to generate the desired results.}
% }
% \label{fig:restrictive}
% \end{subfigure}
\caption{\textbf{Qualitative comparisons.} 
The comparison results prove that our method outperforms the baselines. 
On the left, the figure shows the performance of our method compared to the baseline under the same prompts. The right part of the figure displays the results of the baseline method under restrictive prompts.
}
\label{fig:restrictive}
\label{fig:qualitative}
\label{fig:exp}
\end{figure*}

==> contents/editing/editing.tex <==
\begin{figure*}
\begin{center}
\setlength\tabcolsep{1em}
% \newcommand{\mywidth}{0.2 \textwidth}
\newcommand{\mywidth}{0.22 \linewidth}
\subfloat[Original Image]{\includegraphics[width=\mywidth]{contents/editing/orig.png}}
\hfill
\subfloat[\small \augiefamily A patterned texture that embodies a contemporary and abstract aesthetic]{
\includegraphics[width=\mywidth]{contents/editing/edit1.png}
}
\hfill
\subfloat[\small \augiefamily A pattern of interconnected hexagons]{\includegraphics[width=\mywidth]{contents/editing/edit3.png}}
\hfill
\subfloat[\small \augiefamily A pattern of intertwined swirling and curling designs]{\includegraphics[width=\mywidth]{contents/editing/edit4.png}}
% \begin{tabular}{p{\mywidth}p{\mywidth}p{\mywidth}p{\mywidth}}
% \includegraphics[width=\mywidth]{contents/editing/orig.png}
% & \includegraphics[width=\mywidth]{contents/editing/edit1.png}
% & \includegraphics[width=\mywidth]{contents/editing/edit3.png}
% & \includegraphics[width=\mywidth]{contents/editing/edit4.png}\\
% \quad Original image
% & {\small \augiefamily A patterned texture that embodies a contemporary and abstract aesthetic} 
% & {\small \augiefamily A pattern of interconnected hexagons}  
% & {\small \augiefamily A pattern of intertwined swirling and curling designs} 
% \end{tabular}

\vspace{-1em}
\end{center}

\captionsetup{font={normalsize}} 
\caption{\textbf{Downstream editing resutls.}
% We can perform material editing on generated material. 使用GPT-4模型和预先设定好的api可以让用户使用textual prompt来编辑材质。
We perform material editing on generated material. The user can edit the material using textual prompts through the GPT-4 and the a set of predifined APIs. The corresponding {\augiefamily textual prompts} are shown in {\augiefamily Augie fonts}.
\rh{[replace with different shapes. ]}
}
\label{fig:edit}
\end{figure*}

    


==> contents/editing_method/fx.tex <==
\begin{figure*}
\begin{center}
\setlength\tabcolsep{0.2em}
\newcommand{\mywidth}{\textwidth}
\includegraphics[width=\mywidth]{contents/editing_method/fx.png}
\vspace{-1em}
\end{center}

\captionsetup{font={normalsize}} 
\caption{
\textbf{An example of the filter.} 
% 通过使用这种filter，我们可以直接替换filter input的mask和base material，输出各种各样的效果。
We can replace the mask and base material of the filter input, which can yield various results.
}
\label{fig:fx}
\end{figure*}

    


==> contents/material_class/material_class.tex <==
\begin{figure}
\begin{center}

\newcommand{\mywidth}{0.17 \textwidth}
\begin{tabular}{ccccc}
% \begin{tabular}{m}
\includegraphics[width=\mywidth]{contents/watertight/chair.png}
&\includegraphics[width=\mywidth]{contents/watertight/chair_ab.png}
&\includegraphics[width=\mywidth]{contents/watertight/chair_so.png}
&\includegraphics[width=\mywidth]{contents/watertight/chair_sm.png}
&\includegraphics[width=\mywidth]{contents/watertight/chair_rgb.png}
\\
Generated image & Albedo & Segments & Material Groups & Results
\end{tabular}
\vspace{-1em}
\end{center}

\captionsetup{font={normalsize}} 
\caption{\textbf{Material classification.} 
We show our viusal prompt and the results of material classification.
}
\label{fig:material_class}
\end{figure}

    


==> contents/method_editing/editing.tex <==
\begin{figure*}
\begin{center}
\setlength\tabcolsep{1em}
% \newcommand{\mywidth}{0.2 \textwidth}
\newcommand{\mywidth}{0.22 \linewidth}
\subfloat[Original Image]{\includegraphics[width=\mywidth]{contents/editing/orig.png}}
\hfill
\subfloat[\small \augiefamily A patterned texture that embodies a contemporary and abstract aesthetic]{
\includegraphics[width=\mywidth]{contents/editing/edit1.png}
}
\hfill
\subfloat[\small \augiefamily A pattern of interconnected hexagons]{\includegraphics[width=\mywidth]{contents/editing/edit3.png}}
\hfill
\subfloat[\small \augiefamily A pattern of intertwined swirling and curling designs]{\includegraphics[width=\mywidth]{contents/editing/edit4.png}}
% \begin{tabular}{p{\mywidth}p{\mywidth}p{\mywidth}p{\mywidth}}
% \includegraphics[width=\mywidth]{contents/editing/orig.png}
% & \includegraphics[width=\mywidth]{contents/editing/edit1.png}
% & \includegraphics[width=\mywidth]{contents/editing/edit3.png}
% & \includegraphics[width=\mywidth]{contents/editing/edit4.png}\\
% \quad Original image
% & {\small \augiefamily A patterned texture that embodies a contemporary and abstract aesthetic} 
% & {\small \augiefamily A pattern of interconnected hexagons}  
% & {\small \augiefamily A pattern of intertwined swirling and curling designs} 
% \end{tabular}

\vspace{-1em}
\end{center}

\captionsetup{font={normalsize}} 
\caption{\textbf{Downstream editing.}
% We can perform material editing on generated material. 使用GPT-4模型和预先设定好的api可以让用户使用textual prompt来编辑材质。
We perform material editing on generated material. The user can edit the material using textual prompts through the GPT-4 and the a set of predifined APIs. The corresponding {\augiefamily textual prompts} are shown in {\augiefamily Augie fonts}.
\rh{[Need to add some technical details. ]}
}
\label{fig:edit}
\end{figure*}

    


==> contents/watertight/wtm.tex <==
\begin{figure}
\begin{center}
\iffalse
\setlength\tabcolsep{0.2em}
\newcommand{\mywidth}{0.17 \textwidth}
\begin{tabular}{ccccc}
% \begin{tabular}{m}
\includegraphics[width=\mywidth]{contents/watertight/chair.png}
&\includegraphics[width=\mywidth]{contents/watertight/chair_ab.png}
&\includegraphics[width=\mywidth]{contents/watertight/chair_so.png}
&\includegraphics[width=\mywidth]{contents/watertight/chair_sm.png}
&\includegraphics[width=\mywidth]{contents/watertight/chair_rgb.png}
\\
Generated image & Albedo & Segments & Material Groups & Results
\\
\includegraphics[width=0\mywidth]{contents/watertight/eyeglass_rgb.png}
&\includegraphics[width=\mywidth]{contents/watertight/eyeglass_ab.png}
&\includegraphics[width=\mywidth]{contents/watertight/eyeglass_so.png}
&\includegraphics[width=\mywidth]{contents/watertight/eyeglass_sm.png}
&\includegraphics[width=\mywidth]{contents/watertight/eyeglass.png}
\\
Generated image & Albedo & Segments & Material Groups & Results
\end{tabular}
\fi 
\includegraphics[width=.96\linewidth]{contents/watertight/fig-watertight.pdf}
% \includegraphics[width=.96\linewidth]{contents/watertight/fig-watertight-v2.pdf}
\vspace{-1em}
\end{center}

\captionsetup{font={normalsize}} 
\caption{\textbf{Results on watertight meshes.}
We decompose the watertight mesh into several segments using the graph cut algorithm and generate materials for each segment.}
\label{fig:wtm}
\end{figure}

    


==> shorcuts.tex <==
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bhy}{\hat{\mathbf{y}}}
\newcommand{\bty}{\tilde{\mathbf{y}}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\eye}{\mathbf{I}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bhh}{\hat{\mathbf{h}}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\nR}{\mathbb{R}}
\newcommand{\nN}{\mathbb{N}}
\newcommand{\nL}{\mathbb{L}}
\newcommand{\nF}{\mathbb{F}}
\newcommand{\nS}{\mathbb{S}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cV}{\mathcal{V}}
\def\bgamma{\boldsymbol\gamma}

\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}


% \DeclareMathOperator*{\argmax}{argmax~}
% \DeclareMathOperator*{\argmin}{argmin~}

\renewcommand{\b}{\ensuremath{\mathbf}}

\def\mc{\mathcal}
\def\mb{\mathbf}

\newcommand{\T}{^{\raisemath{-1pt}{\mathsf{T}}}}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{e.g\onedot} \def\Eg{E.g\onedot}
\def\ie{i.e\onedot} \def\Ie{I.e\onedot}
\def\cf{cf\onedot} \def\Cf{Cf\onedot}
\def\etc{etc\onedot} \def\vs{vs\onedot}
\def\wrt{wrt\onedot}
\def\dof{d.o.f\onedot}
% \def\etal{\textit{et~al}\onedot} \def\iid{i.i.d\onedot}
% \def\Fig{Fig\onedot} \def\Eqn{Eqn\onedot} \def\Sec{Sec\onedot} \def\Alg{Alg\onedot}
% \makeatother

\newcommand{\etal}{\textit{et al.}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref*{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\equref}[1]{Eq.~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}

\newcommand\blfootnote[1]{%
\begingroup
\renewcommand\thefootnote{}\footnote{#1}%
\addtocounter{footnote}{-1}%
\endgroup
}

% nice url font and color
\renewcommand\UrlFont{\color{black}\rmfamily}

% rotation
\newcommand*\rot{\rotatebox{90}}
\newcommand{\boldparagraph}[1]{\vspace{0.2cm}\noindent{\bf #1:} }

% horizontally and vertically center align  of table cell
%\newcolumntype{P}[1]{>{\centering\arraybackslash}m{#1}}

% comments
\newif\ifcomment
% set this to show comments
\commenttrue
% set this to hide comments
%\commentfalse
% \ifcomment
% 	\newcommand{\zsz}[1]{ \noindent {\color{blue} {\bf sz:} {#1}} }
%   \newcommand{\yl}[1]{ \noindent {\color{cyan} {\bf yl:} {#1}} }
%   \newcommand{\ctr}[1]{ \noindent {\color{cyan} {\bf ctr:} {#1}} 
%   }
% \else
% \fi

% \newcommand{\red}[1]{\noindent{\color{red}{#1}}}
% \newcommand{\blue}[1]{\noindent{\color{blue}{#1}}}

\newcommand{\tocite}[1]{\textcolor{red}{[TOCITE]}}
\newcommand{\todo}[1]{\textcolor{red}{[TODO: #1]}}


==> tab/ab_corr.tex <==
\begin{table}
    \centering
    \tabcolsep=0.2cm
    \caption{\textbf{Quantitative results of the ablation studies.} 
    % 我们比较我们的方法和其他方法的baseline的PCK和EPE的指标
    We compare our method with baselines in terms of PCK-T and EPE. 
    % PCK
    }
    \begin{threeparttable}
    \begin{tabular}{c c c c c}
    \toprule
    & EPE$\downarrow$    & PCK-1$\uparrow$  & PCK-2$\uparrow$ \\
    \midrule
    Ours         & \textbf{0.72}    & \textbf{0.83}      &\textbf{ 0.99  }      \\
    Ours w/o Lap       & 1.33             & 0.35               & 0.81       \\
    Ours w/o FP     & 1.29             & 0.46              & 0.80         \\
    Ours w/o SFF     & 1.55 & 0.33   & 0.74 \\
    Ours w/o Inv &1.57 &0.37 & 0.65  \\
    SF warping & 1.34             & 0.34              & 0.88          \\
    \bottomrule
    \end{tabular}
    \end{threeparttable}
    \label{ab_corr}
    \vspace{-0.2in}
\end{table}


% \begin{table}
%     \label{tab:comp_dynerf}
%     \resizebox{0.95\columnwidth}{!}{
%     \begin{tabular}{l|c|ccc}
%     \Xhline{3\arrayrulewidth}
%     & Training time (hour) & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$  \\
%     \Xhline{3\arrayrulewidth}
%     \multirow{3}{*}{K-Planes} & 0.8 &  30.78 & 0.953  & 0.218  \\ 
%      & 1.4 & 31.51 & 0.959  & 0.196  \\ 
%      & 2 & \cellsecond 31.61 & \cellsecond 0.961  & \cellfirst 0.182  \\ \hline
%     Ours & 0.5 & \cellfirst 32.81 & \cellfirst 0.972 & \cellsecond 0.195 \\
%     \Xhline{3\arrayrulewidth}
%     \end{tabular}
%     }
%     \end{center}
%     \vspace{-1em}
% \end{table}
 

==> tab/material.tex <==
\begin{table}[t]
    \centering
    \caption{Number of material graphs in various categories.}
    \begin{tabular}{|l|c|}
    \hline
    \textbf{Material Category} & \textbf{Number of Material Graphs} \\ \hline
    Wood                       & 11                                 \\ \hline
    Metal                      & 18                                 \\ \hline
    Plastic                    & 12                                 \\ \hline
    Leather                    & 10                                 \\ \hline
    Fabric                     & 22                                 \\ \hline
    Stone                      & 5                                  \\ \hline
    Ceramic                    & 3                                  \\ \hline
    Rubber                     & 3                                  \\ \hline
    \end{tabular}

\label{tab:material_category}
\end{table}
    
